Study of Rare Nuclear Processes with CUORE

TeO2 bolometers have been used for many years to search for neutrinoless double beta decay in 130-Te. CUORE, a tonne-scale TeO2 detector array, recently published the most sensitive limit on the half-life, $T_{1/2}^{0\nu} > 1.5 \times 10^{25}\,$yr, which corresponds to an upper bound of $140-400$~meV on the effective Majorana mass of the neutrino. While it makes CUORE a world-leading experiment looking for neutrinoless double beta decay, it is not the only study that CUORE will contribute to in the field of nuclear and particle physics. As already done over the years with many small-scale experiments, CUORE will investigate both rare decays (such as the two-neutrino double beta decay of 130-Te and the hypothesized electron capture in 123-Te), and rare processes (e.g., dark matter and axion interactions). This paper describes some of the achievements of past experiments that used TeO2 bolometers, and perspectives for CUORE.

==> authorIJMPA.tex <==
\author{C.~Alduino}
\affiliation{Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA}

\author{K.~Alfonso}
\affiliation{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}

\author{F.~T.~Avignone~III}
\affiliation{Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA}

\author{O.~Azzolini}
\affiliation{INFN -- Laboratori Nazionali di Legnaro, Legnaro (Padova) I-35020, Italy}

\author{G.~Bari}
\affiliation{INFN -- Sezione di Bologna, Bologna I-40127, Italy}

\author{F.~Bellini}
\affiliation{Dipartimento di Fisica, Sapienza Universit\`{a} di Roma, Roma I-00185, Italy}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{G.~Benato}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}

\author{A.~Bersani}
\affiliation{INFN -- Sezione di Genova, Genova I-16146, Italy}

\author{M.~Biassoni}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{A.~Branca}
\affiliation{INFN -- Sezione di Padova, Padova I-35131, Italy}
\affiliation{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}

\author{C.~Brofferio}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{C.~Bucci}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}

\author{A.~Camacho}
\affiliation{INFN -- Laboratori Nazionali di Legnaro, Legnaro (Padova) I-35020, Italy}

\author{A.~Caminata}
\affiliation{INFN -- Sezione di Genova, Genova I-16146, Italy}

\author{L.~Canonica}
\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}

\author{X.~G.~Cao}
\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800, China}

\author{S.~Capelli}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{L.~Cappelli}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}

\author{L.~Cardani}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{P.~Carniti}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{N.~Casali}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{L.~Cassina}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{D.~Chiesa}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{N.~Chott}
\affiliation{Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA}

\author{M.~Clemenza}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{S.~Copello}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Genova, Genova I-16146, Italy}
\affiliation{INFN -- Sezione di Genova, Genova I-16146, Italy}

\author{C.~Cosmelli}
\affiliation{Dipartimento di Fisica, Sapienza Universit\`{a} di Roma, Roma I-00185, Italy}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{O.~Cremonesi}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{R.~J.~Creswick}
\affiliation{Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA}

\author{J.~S.~Cushman}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, CT 06520, USA}

\author{A.~D'Addabbo}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}

\author{D.~D'Aguanno}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}
\affiliation{Dipartimento di Ingegneria Civile e Meccanica, Universit\`{a} degli Studi di Cassino e del Lazio Meridionale, Cassino I-03043, Italy}

\author{I.~Dafinei}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{C.~J.~Davis}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, CT 06520, USA}

\author{S.~Dell'Oro}
\affiliation{Center for Neutrino Physics, Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, USA}

\author{M.~M.~Deninno}
\affiliation{INFN -- Sezione di Bologna, Bologna I-40127, Italy}

\author{S.~Di~Domizio}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Genova, Genova I-16146, Italy}
\affiliation{INFN -- Sezione di Genova, Genova I-16146, Italy}

\author{M.~L.~Di~Vacri}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}
\affiliation{Dipartimento di Scienze Fisiche e Chimiche, Universit\`{a} dell'Aquila, L'Aquila I-67100, Italy}

\author{V.~Domp\`{e}}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}
\affiliation{INFN -- Gran Sasso Science Institute, L'Aquila I-67100, Italy}

\author{A.~Drobizhev}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}

\author{D.~Q.~Fang}
\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800, China}

\author{M.~Faverzani}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{E.~Ferri}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{F.~Ferroni}
\affiliation{Dipartimento di Fisica, Sapienza Universit\`{a} di Roma, Roma I-00185, Italy}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{E.~Fiorini}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}

\author{M.~A.~Franceschi}
\affiliation{INFN -- Laboratori Nazionali di Frascati, Frascati (Roma) I-00044, Italy}

\author{S.~J.~Freedman\footnote{Deceased}}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}

\author{B.~K.~Fujikawa}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}

\author{A.~Giachero}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{L.~Gironi}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{A.~Giuliani}
\affiliation{CSNSM, Univ. Paris-Sud, CNRS/IN2P3, Université Paris-Saclay, 91405 Orsay, France}

\author{L.~Gladstone}
\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{P.~Gorla}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}

\author{C.~Gotti}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{T.~D.~Gutierrez}
\affiliation{Physics Department, California Polytechnic State University, San Luis Obispo, CA 93407, USA}

\author{K.~Han}
\affiliation{INPAC and School of Physics and Astronomy, Shanghai Jiao Tong University; Shanghai Laboratory for Particle Physics and Cosmology, Shanghai 200240, China}

\author{K.~M.~Heeger}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, CT 06520, USA}

\author{R.~Hennings-Yeomans}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}

\author{H.~Z.~Huang}
\affiliation{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}

\author{G.~Keppel}
\affiliation{INFN -- Laboratori Nazionali di Legnaro, Legnaro (Padova) I-35020, Italy}

\author{Yu.~G.~Kolomensky}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}

\author{A.~Leder}
\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{C.~Ligi}
\affiliation{INFN -- Laboratori Nazionali di Frascati, Frascati (Roma) I-00044, Italy}

\author{K.~E.~Lim}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, CT 06520, USA}

\author{Y.~G.~Ma}
\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800, China}

\author{L.~Marini}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Genova, Genova I-16146, Italy}
\affiliation{INFN -- Sezione di Genova, Genova I-16146, Italy}

\author{M.~Martinez}
\affiliation{Dipartimento di Fisica, Sapienza Universit\`{a} di Roma, Roma I-00185, Italy}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}
\affiliation{Laboratorio de Fisica Nuclear y Astroparticulas, Universidad de Zaragoza, Zaragoza 50009, Spain}

\author{R.~H.~Maruyama}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, CT 06520, USA}

\author{Y.~Mei}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}

\author{N.~Moggi}
%\affiliation{Dipartimento di Fisica e Astronomia, Alma Mater Studiorum -- Universit\`{a} di Bologna, Bologna I-40127, Italy}
\affiliation{Dipartimento di Fisica e Astronomia, Alma Mater Studiorum -- Universit\`{a} di Bologna}
\affiliation{INFN -- Sezione di Bologna, Bologna I-40127, Italy}

\author{S.~Morganti}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{S.~S.~Nagorny}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}
\affiliation{INFN -- Gran Sasso Science Institute, L'Aquila I-67100, Italy}

\author{T.~Napolitano}
\affiliation{INFN -- Laboratori Nazionali di Frascati, Frascati (Roma) I-00044, Italy}

\author{M.~Nastasi}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{C.~Nones}
\affiliation{Service de Physique des Particules, CEA / Saclay, 91191 Gif-sur-Yvette, France}

\author{E.~B.~Norman}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA}
\affiliation{Department of Nuclear Engineering, University of California, Berkeley, CA 94720, USA}

\author{V.~Novati}
\affiliation{CSNSM, Univ. Paris-Sud, CNRS/IN2P3, Université Paris-Saclay, 91405 Orsay, France}

\author{A.~Nucciotti}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{I.~Nutini}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}
\affiliation{INFN -- Gran Sasso Science Institute, L'Aquila I-67100, Italy}

\author{T.~O'Donnell}
\affiliation{Center for Neutrino Physics, Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, USA}

\author{J.~L.~Ouellet}
\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{C.~E.~Pagliarone}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}
%\affiliation{Dipartimento di Ingegneria Civile e Meccanica, Universit\`{a} degli Studi di Cassino e del Lazio Meridionale, Cassino I-03043, Italy}
\affiliation{Universit\`{a} degli Studi di Cassino e del Lazio Meridionale, Cassino I-03043, Italy}

\author{M.~Pallavicini}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Genova, Genova I-16146, Italy}
\affiliation{INFN -- Sezione di Genova, Genova I-16146, Italy}

\author{V.~Palmieri}
\affiliation{INFN -- Laboratori Nazionali di Legnaro, Legnaro (Padova) I-35020, Italy}

\author{L.~Pattavina}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}

\author{M.~Pavan}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{G.~Pessina}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{C.~Pira}
\affiliation{INFN -- Laboratori Nazionali di Legnaro, Legnaro (Padova) I-35020, Italy}

\author{S.~Pirro}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}

\author{S.~Pozzi}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{E.~Previtali}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{F.~Reindl}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{C.~Rosenfeld}
\affiliation{Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA}

\author{C.~Rusconi}
%\affiliation{Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA}
\affiliation{University of South Carolina, Columbia, SC 29208, USA}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}

\author{M.~Sakai}
\affiliation{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}

\author{S.~Sangiorgio}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA}

\author{D.~Santone}
\affiliation{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}
\affiliation{Dipartimento di Scienze Fisiche e Chimiche, Universit\`{a} dell'Aquila, L'Aquila I-67100, Italy}

\author{B.~Schmidt}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}

\author{J.~Schmidt}
\affiliation{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}

\author{N.~D.~Scielzo}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA}

\author{V.~Singh}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}

\author{M.~Sisti}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{L.~Taffarello}
\affiliation{INFN -- Sezione di Padova, Padova I-35131, Italy}

\author{F.~Terranova}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{C.~Tomei}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{M.~Vignati}
\affiliation{INFN -- Sezione di Roma, Roma I-00185, Italy}

\author{S.~L.~Wagaarachchi}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}

\author{B.~S.~Wang}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA}
\affiliation{Department of Nuclear Engineering, University of California, Berkeley, CA 94720, USA}

\author{H.~W.~Wang}
\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800, China}

\author{B.~Welliver}
\affiliation{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}

\author{J.~Wilson}
\affiliation{Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA}

\author{K.~Wilson}
\affiliation{Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA}

\author{L.~A.~Winslow}
\affiliation{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{T.~Wise}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, CT 06520, USA}
\affiliation{Department of Physics, University of Wisconsin, Madison, WI 53706, USA}

\author{L.~Zanotti}
\affiliation{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\affiliation{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}

\author{G.~Q.~Zhang}
\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800, China}

\author{S.~Zimmermann}
\affiliation{Engineering Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}

\author{S.~Zucchelli}
\affiliation{Dipartimento di Fisica e Astronomia, Alma Mater Studiorum -- Universit\`{a} di Bologna, Bologna I-40127, Italy}
\affiliation{INFN -- Sezione di Bologna, Bologna I-40127, Italy}
